Playing Pushdown Parity Games in a Hurry

We continue the investigation of finite-duration variants of infinite-duration games by extending known results for games played on finite graphs to those played on infinite ones. In particular, we establish an equivalence between pushdown parity games and a finite-duration variant. This allows us to determine the winner of a pushdown parity game by solving a reachability game on a finite tree.

==> eptcsdata.tex <==
\providecommand{\firstpage}{183}
\providecommand{\publicationstatus}{M. Faella, A. Murano (Eds.): Games, Automata, Logics\\
and Formal Verification (GandALF 2012)\\
EPTCS 96, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.96.14}{10.4204/EPTCS.96.14}}

